Local Hamiltonians in Quantum Computation

In this thesis, I investigate aspects of local Hamiltonians in quantum computing. First, I focus on the Adiabatic Quantum Computing model, based on evolution with a time dependent Hamiltonian. I show that to succeed using AQC, the Hamiltonian involved must have local structure, which leads to a result about eigenvalue gaps from information theory. I also improve results about simulating quantum circuits with AQC. Second, I look at classically simulating time evolution with local Hamiltonians and finding their ground state properties. I give a numerical method for finding the ground state of translationally invariant Hamiltonians on an infinite tree. This method is based on imaginary time evolution within the Matrix Product State ansatz, and uses a new method for bringing the state back to the ansatz after each imaginary time step. I then use it to investigate the phase transition in the transverse field Ising model on the Bethe lattice. Third, I focus on locally constrained quantum problems Local Hamiltonian and Quantum Satisfiability and prove several new results about their complexity. Finally, I define a Hamiltonian Quantum Cellular Automaton, a continuous-time model of computation which doesn't require control during the computation process, only preparation of product initial states. I construct two of these, showing that time evolution with a simple, local, translationally invariant and time-independent Hamiltonian can be used to simulate quantum circuits.

==> unused-lineends.tex <==
% unused - walk on a line with boundary terms.

\section{Quantum Walk on a Line with Extra Boundary Terms}
\label{endsline}

Here I investigate the quantum walk on a line of length $L$ governed by the Hamiltonian \eqref{H1hamiltonian} with additional boundary terms.
\begin{eqnarray}
	H_{ends} = 
	- \left(\ket{1}\bra{1} + \ket{L}\bra{L}\right)
	- \sum_{j=1}^{L-1} 
	\left(\ket{j}\bra{j+1} + \ket{j+1}\bra{j}\right).
	\label{Hendhamiltonian}
\end{eqnarray}
This Hamiltonian is the nontrivial part of Kitaev's propagation Hamiltonian $H_{prop} = \ii + \half H_{ends}$ (see Appendix \ref{appProp}) and is thus responsible for its dynamics.
I also use \eqref{Hendhamiltonian} in Section \ref{ch4:train} for my {\em train switch} Hamiltonian Computer.

Its eigenvectors are plain waves
with momenta and eigenvalues
\begin{eqnarray}
	p_j &=& \frac{\pi (j-1)}{L}, \\
	\lambda_j &=& - 2 \cos \left(p_j\right),
	\label{endseigenval}
\end{eqnarray}
for $j=1,\dots,L$. The eigenvectors 
$\kets{\phi^{(j)}} = \sum_{k=1}^{L} \phi^{(j)}_k \ket{k}$ are given by
\begin{eqnarray}
	\phi^{(1)}_k &=& \sqrt{\frac{1}{L}}, 
\end{eqnarray}
and
\begin{eqnarray}
	\phi^{(j>1)}_k &=& \sqrt{\frac{2}{L+1}} \, 
		\cos \left( p_j \left( k-\half \right) \right).
	\label{endseigenvec}
\end{eqnarray}

The analysis of the dynamics of this walk follows the mold of Section \ref{plainline}. I want to show how fast the probability distribution converges to the limiting distribution, when starting in the state $\ket{k=0}$. Because all the eigenvalues of $H_{ends}$ are distinct, the limiting distribution is given by \eqref{deflimdistrib}, which in this case results in 
\begin{eqnarray}
	\pi(m|c) 
	 = \frac{L-1}{L^2} + 
	 	+ \frac{\delta_{m,c} + \delta_{m,L+1-c}}{2L}.
	 \label{Pendslimiting}
\end{eqnarray}
Lemma \ref{linelemma} of Section \ref{plainline} reformulated for the modified walk on a line is
\begin{lem5x}
Consider a modified continuous time quantum walk on a line of length $L$, with the Hamiltonian given by \eqref{Hendhamiltonian}. Let the system evolve for time $\tau \leq \tau_{ends}$ chosen uniformly at random, starting in a position basis state $\ket{c}$.
The average probability distribution $p_{\tau_{ends}}(\cdot|c)$ converges to the limiting probability distribution $\pi(\cdot|c)$ as
\begin{eqnarray}
	\sum_{m=1}^{L} \left| \bar{p}_{\tau_{ends}}(m|c) - \pi(m|c) \right|
	\leq 
		O\left(\frac{L}{\tau_{ends}}\right).
	\label{limitinglemmax}
\end{eqnarray}
\end{lem5x}
The proof follows the proof of Lemma \ref{convergelemma} in Section \ref{plainline}. The modified and generalized Lemma \ref{linelemma} then reads
\begin{lem4x}
Consider a modified continuous time quantum walk on a line of length $L$, with the Hamiltonian given by \eqref{Hendhamiltonian}. Let the system evolve for a time $\tau \leq \tau_{ends}$ chosen uniformly at random, starting in a position basis state $\ket{c}$.
The probability to measure a state $\ket{t}$ with $t>(1-q)L$ is then bounded from below as $p_{ends}\geq q-O\left(\frac{L}{\tau_{ends}}\right)$. 
\end{lem4x}
Its proof again follows the proof of Lemma \ref{linelemma} given in Section \ref{plainline}.





% unused - quantum walk on a circle

